Top Quark Modelling and Tuning at CMS

Recent measurements dedicated to improving the understanding of modelling top quark pair (${\text{t}\overline{\text{t}}}$) production at the LHC are summarised. These measurements, performed with proton-proton collision data collected by the CMS detector at $\sqrt{s}=$ 13 TeV, probe the underlying event in ${\text{t}\overline{\text{t}}}$ events, and use the abundance of jets in ${\text{t}\overline{\text{t}}}$ events to study the substructure of jets. A new set of tunes for PYTHIA 8, and their performance with ${\text{t}\overline{\text{t}}}$ data, are also discussed.

==> econfmacros.tex <==


%%%  useful macros for econf proceedings articles:
\RequirePackage{xspace}
\RequirePackage{amsmath}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%  basic formatting macros:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  single-line equations:

% \def\beq{\begin{equation}}
% \def\eeq#1{\label{#1}\end{equation}}
% \def\eeqn{\end{equation}}

% %%  multiple-line equations  (use \CR as the carriage return):

% \def\beqa{\begin{eqnarray}}
% \def\eeqa#1{\label{#1}\end{eqnarray}}
% \def\eeqan{\end{eqnarray}}
% \def\CR{\nonumber \\ }

% %%  reference to an equation number:

% \def\leqn#1{(\ref{#1})}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  bibliographic entries   (use this or the SPIRES LaTeX output)

% %%   Journal or bibliographic formatting macros are obsolete!
% %%   The SLAC/SPIRES database supplies properly formatted citations;
% %%      click on  LaTeX(US) or LaTeX(EU)   

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  sizing and bars

% \def\st{\scriptstyle}
% \def\sst{\scriptscriptstyle}

% \def\overbar#1{\overline{#1}}
% \let\littlebar=\bar
% \let\bar=\overbar

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  text-mode macros:

% \def\etal{{\it et al.}}
% \def\ie{{\it i.e.}}
% \def\eg{{\it e.g.}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  expectation values:

% \def\VEV#1{\left\langle{ #1} \right\rangle}
% \def\bra#1{\left\langle{ #1} \right|}
% \def\ket#1{\left| {#1} \right\rangle}
% \def\vev#1{\langle #1 \rangle}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  caligraphic letters (for matrix elements, luminosity, etc.)

% \def\D{{\cal D}}
% \def\L{{\cal L}}
% \def\M{{\cal M}}
% \def\O{{\cal O}}
% \def\W{{\cal W}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  matrix operations and fractions:

% \def\One{{\bf 1}}
% \def\hc{{\mbox{\rm h.c.}}}
% \def\tr{{\mbox{\rm tr}}}
% \def\half{\frac{1}{2}}
% \def\thalf{\frac{3}{2}}
% \def\third{\frac{1}{3}}
% \def\tthird{\frac{2}{3}}

% \def\Dslash{\not{\hbox{\kern-4pt $D$}}}
% \def\dslash{\not{\hbox{\kern-2pt $\del$}}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  high-energy physics terminology:

% \def\Pl{{\mbox{\scriptsize Pl}}}
% \def\eff{{\mbox{\scriptsize eff}}}
% \def\CM{{\mbox{\scriptsize CM}}}
% \def\BR{\mbox{\rm BR}}
% \def\ee{e^+e^-}
% \def\sstw{\sin^2\theta_w}
% \def\cstw{\cos^2\theta_w}
% \def\mz{m_Z}
% \def\gz{\Gamma_Z}
% \def\mw{m_W}
% \def\mt{m_t}
% \def\gt{\Gamma_t}
% \def\mh{m_h}
% \def\gmu{G_\mu}
% \def\GF{G_F}
% \def\alphas{\alpha_s}
% \def\msb{{\bar{\ssstyle M \kern -1pt S}}}
% \def\lmsb{\Lambda_{\msb}}
% \def\ELER{e^-_Le^+_R}
% \def\EREL{e^-_Re^+_L}
% \def\ELEL{e^-_Le^+_L}
% \def\ERER{e^-_Re^+_R}
% \def\eps{\epsilon}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%  supersymmetry:

% \def\ch#1{\widetilde\chi^+_{#1}}
% \def\chm#1{\widetilde\chi^-_{#1}}
% \def\neu#1{\widetilde\chi^0_{#1}}
% \def\s#1{\widetilde{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\newcommand{\PYTHIA} {{\textsc{pythia 8}}\xspace}
\newcommand{\HERWIGS} {{\textsc{herwig 7}}\xspace}
\newcommand{\SHERPA} {{\textsc{sherpa}}\xspace}
\newcommand{\MG} {\textsc{MadGraph\_mc@nlo}\xspace}
\newcommand{\DIRE} {\textsc{dire}\xspace}

\newcommand{\ttbar}{\ensuremath{{\text{t}\overline{\text{t}}}}\xspace}
\newcommand{\topmass}{\ensuremath{m_{\mathrm{t}}}\xspace}

\providecommand{\epm}{\ensuremath{e^\pm}\xspace} % electron
\providecommand{\mupm}{\ensuremath{\mu^\pm}\xspace} % muon

\providecommand{\bJet}{\ensuremath{b}-jet\xspace} % b jet

\newcommand{\POWHEG} {{\textsc{powheg}}\xspace}

\newcommand{\POWHEGPYTHIA} {{\textsc{powheg+pythia 8}}\xspace}


\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\ptbar}{\ensuremath{|\overline{p}_{\mathrm{T}}|}\xspace}
\newcommand{\llmass}{\ensuremath{m_{\mathrm{ll}}}\xspace}
\newcommand{\ptllvec}{\ensuremath{\vec{p_{\mathrm{ll}}}}\xspace}

\newcommand{\deltaPhi}{\ensuremath{\Delta\Phi}\xspace}

\newcommand{\fbinv} {\mbox{\ensuremath{\,\text{fb}^\text{$-$1}}}\xspace}

\newcommand{\alpsfsr}{\ensuremath{\alpha_\mathrm{S}^{\mathrm{FSR}}\left(\mathrm{M}_\mathrm{Z}\right)}\xspace}
\newcommand{\alpS}{\ensuremath{\alpha_S}\xspace}

\providecommand{\chis}{\ensuremath{\chi^2}\xspace}

\newcommand{\deltaRg}{\ensuremath{\Delta{R_g}}\xspace}

\newcommand{\cuettune}{\textsc{CUETP8M2T4}\xspace}
\newcommand{\oldcuettune}{\textsc{CUETP8M1}\xspace}

\newcommand{\sqrts}{\ensuremath{\sqrt{\smash[b]{s}}}\xspace}
\newcommand{\TeV}{\ensuremath{\,\text{Te\hspace{-.08em}V}}\xspace}
